Benchmarking the flow of epithelial cell monolayer with self-aligning deformable active membranes

Collective cell migration emerges from the interplay between motility, deformability and mechanical interactions, yet incorporating these ingredients into computationally efficient tissue models remains challenging. Here, we benchmark self-aligning deformable active membranes in a confined-flow geometry that mimics epithelial monolayer migration around a circular obstacle. In this model, cells are represented as deformable, adhesive membranes whose self-propulsion direction relaxes towards their velocity. By systematically varying the self-alignment timescale, cell-cell adhesion and inlet forcing, we characterize the resulting flows through collective alignment, relative density, neighbor rearrangements and spatial velocity fields. The model captures a broad spectrum of tissue behaviors, ranging from disordered, liquid-like flows to highly aligned, solid-like states. Compared with a related multiparticle model, self-aligning active membranes achieve stronger collective alignment, exhibit a more systematic density response and access states closer to both limits of the solid-liquid spectrum. We further show that increasing the target shape index promotes cell elongation and accelerates tissue flow, directly linking cell-scale deformability to tissue-scale transport. Finally, we compare simulated velocity profiles with experimental measurements from in vitro migrating MDCK epithelial cell monolayers and find qualitative agreement across multiple horizontal and vertical transects around the obstacle. These results establish self-aligning deformable active membranes as a versatile framework for connecting cell mechanics, shape adaptation and self-alignment to collective tissue migration in confined geometries.

==> main_labels.tex <==
\newlabel{fig:melina}{{1a}{2}{Experiment}{figure.caption.1}{}}
\newlabel{fig:melina@cref}{{[subfigure][1][1]1a}{[1][1][]2}{}{}{}}
\newlabel{sub@fig:melina}{{a}{2}{Experiment}{figure.caption.1}{}}
\newlabel{sub@fig:melina@cref}{{[subfigure][1][1]1a}{[1][1][]2}{}{}{}}
\newlabel{fig:channel_view_rings}{{1b}{2}{Simulation}{figure.caption.1}{}}
\newlabel{fig:channel_view_rings@cref}{{[subfigure][2][1]1b}{[1][1][]2}{}{}{}}
\newlabel{sub@fig:channel_view_rings}{{b}{2}{Simulation}{figure.caption.1}{}}
\newlabel{sub@fig:channel_view_rings@cref}{{[subfigure][2][1]1b}{[1][1][]2}{}{}{}}
\newlabel{fig:model_pol_scheme}{{1c}{2}{Self-alignment}{figure.caption.1}{}}
\newlabel{fig:model_pol_scheme@cref}{{[subfigure][3][1]1c}{[1][1][]2}{}{}{}}
\newlabel{sub@fig:model_pol_scheme}{{c}{2}{Self-alignment}{figure.caption.1}{}}
\newlabel{sub@fig:model_pol_scheme@cref}{{[subfigure][3][1]1c}{[1][1][]2}{}{}{}}
\newlabel{fig:model_scheme}{{1d}{2}{Forces}{figure.caption.1}{}}
\newlabel{fig:model_scheme@cref}{{[subfigure][4][1]1d}{[1][1][]2}{}{}{}}
\newlabel{sub@fig:model_scheme}{{d}{2}{Forces}{figure.caption.1}{}}
\newlabel{sub@fig:model_scheme@cref}{{[subfigure][4][1]1d}{[1][1][]2}{}{}{}}
\newlabel{fig:fig1}{{1}{2}{Model used to simulate epithelial monolayer migration in Stokes flow. Panel~(\subref {fig:melina}) shows a snapshot acquired during the experimental procedure of Duprez and colleagues~\cite {duprez2026geometric}. Panel~(\subref {fig:channel_view_rings}) shows a channel filled with active membranes. Membranes are colored by their asphericity, a scalar measure of shape anisotropy ranging from 0 for more circular membranes (dark purple) to 1 for more elongated membranes (yellow). Insets show magnified views of the channel region immediately before and after the obstacle. Panels~(\subref {fig:model_pol_scheme}) and (\subref {fig:model_scheme}) illustrate two interacting active membranes, labeled $j$ and $k$. Each membrane is depicted as a sequence of particles of diameter $\sigma $ [\cref {eq:energy_c_adh}], shown as circles of the same color, with black lines representing the springs connecting neighboring particles. Panel~(\subref {fig:model_pol_scheme}) illustrates the self-alignment mechanism: the membrane polarization $\mathbf {\hat n}$ relaxes toward the direction of the membrane velocity $\mathbf {\hat v}$ over the characteristic timescale $\tau $ [\cref {eq:eq_motion}]. Panel~(\subref {fig:model_scheme}) illustrates the forces acting on the particles. Orange arrows represent spring forces [\cref {eq:energy_p}], green arrows represent forces arising from the preferred-area energy [\cref {eq:energy_a}], and blue arrows represent interparticle interactions [\cref {eq:energy_c_adh}]}{figure.caption.1}{}}
\newlabel{fig:fig1@cref}{{[figure][1][]1}{[1][1][]2}{}{}{}}
\newlabel{fig:channel_view}{{2}{3}{Illustration of the channel geometry, with dimensions expressed in units of the equilibrium membrane diameter $d_{eq}$ [\cref {eq:ring_diamenter_eq}]. The green region indicates where membranes are created, the red region where they are removed, the yellow region denotes the input measurement region, and the purple region denotes the output measurement region. The black circle represents the obstacle}{figure.caption.2}{}}
\newlabel{fig:channel_view@cref}{{[figure][2][]2}{[1][2][]3}{}{}{}}
\newlabel{sec:model}{{2}{3}{Model}{section.2}{}}
\newlabel{sec:model@cref}{{[section][2][]2}{[1][3][]3}{}{}{}}
\newlabel{eq:eq_motion}{{1}{3}{Model}{equation.1}{}}
\newlabel{eq:eq_motion@cref}{{[equation][1][]1}{[1][3][]3}{}{}{}}
\newlabel{eq:energy}{{2}{3}{Model}{equation.2}{}}
\newlabel{eq:energy@cref}{{[subequation][0][2]2}{[1][3][]3}{}{}{}}
\newlabel{eq:energy_p}{{2a}{3}{Model}{equation.2a}{}}
\newlabel{eq:energy_p@cref}{{[subequation][1][2]2a}{[1][3][]3}{}{}{}}
\newlabel{eq:energy_a}{{2b}{3}{Model}{equation.2b}{}}
\newlabel{eq:energy_a@cref}{{[subequation][2][2]2b}{[1][3][]3}{}{}{}}
\newlabel{eq:energy_c_adh}{{2c}{3}{Model}{equation.2c}{}}
\newlabel{eq:energy_c_adh@cref}{{[subequation][3][2]2c}{[1][3][]3}{}{}{}}
\newlabel{eq:energy_total}{{2d}{3}{Model}{equation.2d}{}}
\newlabel{eq:energy_total@cref}{{[subequation][4][2]2d}{[1][3][]3}{}{}{}}
\newlabel{sec:stokes}{{3}{4}{Stokes geometry system}{section.3}{}}
\newlabel{sec:stokes@cref}{{[section][3][]3}{[1][4][]4}{}{}{}}
\newlabel{eq:ring_diamenter_eq}{{3}{4}{Stokes geometry system}{equation.3}{}}
\newlabel{eq:ring_diamenter_eq@cref}{{[equation][3][]3}{[1][4][]4}{}{}{}}
\newlabel{eq:obs_force}{{4}{4}{Boundary conditions in the transverse direction and at the obstacle}{equation.4}{}}
\newlabel{eq:obs_force@cref}{{[equation][4][]4}{[1][4][]4}{}{}{}}
\newlabel{tab:fix_pars}{{1}{4}{Fixed parameters used in all simulations. Length, time, and energy are measured in units of $\sigma $, $\tau _0=\sigma /v_0$, and $\epsilon = v_0\sigma /\mu $, respectively. Parameters marked as “Ref. unit” define the system of units employed throughout this work}{table.caption.3}{}}
\newlabel{tab:fix_pars@cref}{{[table][1][]1}{[1][4][]4}{}{}{}}
\newlabel{sec:exploration}{{4}{4}{Exploration method}{section.4}{}}
\newlabel{sec:exploration@cref}{{[section][4][]4}{[1][4][]4}{}{}{}}
\newlabel{fig:low_align_snaps}{{3a}{5}{High $\tau $}{figure.caption.4}{}}
\newlabel{fig:low_align_snaps@cref}{{[subfigure][1][3]3a}{[1][4][]5}{}{}{}}
\newlabel{sub@fig:low_align_snaps}{{a}{5}{High $\tau $}{figure.caption.4}{}}
\newlabel{sub@fig:low_align_snaps@cref}{{[subfigure][1][3]3a}{[1][4][]5}{}{}{}}
\newlabel{fig:high_align_snaps}{{3b}{5}{Low $\tau $}{figure.caption.4}{}}
\newlabel{fig:high_align_snaps@cref}{{[subfigure][2][3]3b}{[1][4][]5}{}{}{}}
\newlabel{sub@fig:high_align_snaps}{{b}{5}{Low $\tau $}{figure.caption.4}{}}
\newlabel{sub@fig:high_align_snaps@cref}{{[subfigure][2][3]3b}{[1][4][]5}{}{}{}}
\newlabel{fig:snapshots_color_vel}{{3}{5}{Simulation snapshots, centered on the obstacle, with membranes colored according to their velocity orientation: angle between the velocity and the $x$ axis. The mapping of angles to colors is illustrated in the color wheel located between the figures}{figure.caption.4}{}}
\newlabel{fig:snapshots_color_vel@cref}{{[figure][3][]3}{[1][4][]5}{}{}{}}
\newlabel{tab:parameter_summary}{{2}{5}{Mapping between the explored parameters, simulation labels, parameter ranges, and associated physical quantities. The label letter is chosen to reflect the physical quantity to which the parameter is related}{table.caption.5}{}}
\newlabel{tab:parameter_summary@cref}{{[table][2][]2}{[1][5][]5}{}{}{}}
\newlabel{sec:measuments}{{5}{5}{Measurements}{section.5}{}}
\newlabel{sec:measuments@cref}{{[section][5][]5}{[1][5][]5}{}{}{}}
\newlabel{eq:input_alignment}{{7}{5}{Input measurements}{equation.7}{}}
\newlabel{eq:input_alignment@cref}{{[equation][7][]7}{[1][5][]5}{}{}{}}
\newlabel{fig:low_align_output_vel}{{4a}{6}{High $\tau $}{figure.caption.6}{}}
\newlabel{fig:low_align_output_vel@cref}{{[subfigure][1][4]4a}{[1][5][]6}{}{}{}}
\newlabel{sub@fig:low_align_output_vel}{{a}{6}{High $\tau $}{figure.caption.6}{}}
\newlabel{sub@fig:low_align_output_vel@cref}{{[subfigure][1][4]4a}{[1][5][]6}{}{}{}}
\newlabel{fig:high_align_output_vel}{{4b}{6}{Low $\tau $}{figure.caption.6}{}}
\newlabel{fig:high_align_output_vel@cref}{{[subfigure][2][4]4b}{[1][5][]6}{}{}{}}
\newlabel{sub@fig:high_align_output_vel}{{b}{6}{Low $\tau $}{figure.caption.6}{}}
\newlabel{sub@fig:high_align_output_vel@cref}{{[subfigure][2][4]4b}{[1][5][]6}{}{}{}}
\newlabel{fig:vel_output_measurements}{{4}{6}{Velocity fields for all simulated cases. The black circle represents the channel obstacle. The white arrow inside it is a reference velocity vector, with its magnitude indicated above; the arrow scale differs between graphs. Panel \subref {fig:low_align_output_vel} shows the four cases with low alignment and panel \subref {fig:high_align_output_vel} the four cases with high alignment. It is clear that the velocity field is significantly more organized in cases with high alignment compared to those with low alignment and the field is usually symmetric with respect to the $x$-axis, with the only exception being the \case {1}{0}{0}}{figure.caption.6}{}}
\newlabel{fig:vel_output_measurements@cref}{{[figure][4][]4}{[1][5][]6}{}{}{}}
\newlabel{fig:low_align_output_den}{{5a}{6}{High $\tau $}{figure.caption.7}{}}
\newlabel{fig:low_align_output_den@cref}{{[subfigure][1][5]5a}{[1][5][]6}{}{}{}}
\newlabel{sub@fig:low_align_output_den}{{a}{6}{High $\tau $}{figure.caption.7}{}}
\newlabel{sub@fig:low_align_output_den@cref}{{[subfigure][1][5]5a}{[1][5][]6}{}{}{}}
\newlabel{fig:high_align_output_den}{{5b}{6}{Low $\tau $}{figure.caption.7}{}}
\newlabel{fig:high_align_output_den@cref}{{[subfigure][2][5]5b}{[1][5][]6}{}{}{}}
\newlabel{sub@fig:high_align_output_den}{{b}{6}{Low $\tau $}{figure.caption.7}{}}
\newlabel{sub@fig:high_align_output_den@cref}{{[subfigure][2][5]5b}{[1][5][]6}{}{}{}}
\newlabel{fig:den_output_measurements}{{5}{6}{Relative density fields for all simulated cases shown as color maps with values increasing from blue to red. Panel \subref {fig:low_align_output_den} shows the four cases with low alignment and panel \subref {fig:high_align_output_den} the four cases with high alignment. For each panel, the color scale on the right side of each graph indicates the specific scale used, which may differ between graphs. However, graphs in the same position across different panels share the same scale, allowing for easy comparison in cases where only the alignment changes. Note that the lowest value the relative density can have is $-1$, which corresponds to a complete vacuum. The black circle is the channel obstacle. The overall effect of the obstacle is a reduction in density downstream of its location, as indicated by the predominance of blue tones on the right side of the graphs compared to the left. In cases with high adhesion (cases with $T1$ in their labels, i.e., the bottom row in each panel), a vacuum region appears behind the obstacle. The size of this region is influenced by the density parameter, becoming smaller for higher density values (when the case has $D1$ in its label)}{figure.caption.7}{}}
\newlabel{fig:den_output_measurements@cref}{{[figure][5][]5}{[1][5][]6}{}{}{}}
\newlabel{eq:rel_den}{{8}{6}{Input measurements}{equation.8}{}}
\newlabel{eq:rel_den@cref}{{[equation][8][]8}{[1][6][]6}{}{}{}}
\newlabel{eq:delta_i}{{9}{6}{Input measurements}{equation.9}{}}
\newlabel{eq:delta_i@cref}{{[equation][9][]9}{[1][6][]6}{}{}{}}
\newlabel{eq:delta}{{10}{7}{Input measurements}{equation.10}{}}
\newlabel{eq:delta@cref}{{[equation][10][]10}{[1][7][]7}{}{}{}}
\newlabel{tab:all_input_measurements}{{3}{7}{Input measurements for the eight simulated cases, comparing the MPM and the DAMM. Cases are grouped by the alignment parameter $\tau $: the first four rows correspond to low alignment, and the last four to high alignment. Each input measurement—alignment ($\Psi $), relative density ($\delta \rho $), and solid--liquid behavior ($\Delta $)—is presented in a column with two subcolumns, one for each model. Compared to the MPM, the DAMM achieves higher alignment, displays more consistent relative density values, and reaches values closer to the extremes of the solid--liquid spectrum, as discussed in the text}{table.caption.8}{}}
\newlabel{tab:all_input_measurements@cref}{{[table][3][]3}{[1][7][]7}{}{}{}}
\newlabel{fig:snapshots_simulacao}{{6}{8}{Exploration of the shape index $p_0$. Panels (a, b): steady-state simulation snapshots centered on the channel obstacle for $p_0=3.2$ and $p_0=4.0$, respectively. Cells are rounder and more rigid at $p_0=3.2$, whereas they are considerably more deformable at $p_0=4.0$. Cell colors indicate asphericity ($\mathcal {A}$). The inset within the obstacle shows a magnified view of a selected square region of the tissue. Panel (c): effect of cell deformability parameter $p_0$ on tissue velocity ($v_{\uparrow }$) and mean asphericity over all membranes in the channel ($\langle \mathcal {A} \rangle $). Both $v_{\uparrow }$ and $\langle \mathcal {A} \rangle $ increase monotonically with increasing $p_0$, demonstrating that more flexible cells enable faster collective migration through the channel. Error bars represent the standard error of the mean. Panel (d): asphericity distribution ($p(\mathcal {A})$) for all membranes in the channel at the final state, shown for three values of $p_0$. At lower $p_0$, the membranes are predominantly circular, resulting in a pronounced peak at $\mathcal {A}=0$. As $p_0$ increases, the distribution broadens toward larger $\mathcal {A}$, indicating increasingly elongated membrane shapes}{figure.caption.9}{}}
\newlabel{fig:snapshots_simulacao@cref}{{[figure][6][]6}{[1][7][]8}{}{}{}}
\newlabel{fig:small_po}{{6a}{8}{Exploration of the shape index $p_0$. Panels (a, b): steady-state simulation snapshots centered on the channel obstacle for $p_0=3.2$ and $p_0=4.0$, respectively. Cells are rounder and more rigid at $p_0=3.2$, whereas they are considerably more deformable at $p_0=4.0$. Cell colors indicate asphericity ($\mathcal {A}$). The inset within the obstacle shows a magnified view of a selected square region of the tissue. Panel (c): effect of cell deformability parameter $p_0$ on tissue velocity ($v_{\uparrow }$) and mean asphericity over all membranes in the channel ($\langle \mathcal {A} \rangle $). Both $v_{\uparrow }$ and $\langle \mathcal {A} \rangle $ increase monotonically with increasing $p_0$, demonstrating that more flexible cells enable faster collective migration through the channel. Error bars represent the standard error of the mean. Panel (d): asphericity distribution ($p(\mathcal {A})$) for all membranes in the channel at the final state, shown for three values of $p_0$. At lower $p_0$, the membranes are predominantly circular, resulting in a pronounced peak at $\mathcal {A}=0$. As $p_0$ increases, the distribution broadens toward larger $\mathcal {A}$, indicating increasingly elongated membrane shapes}{subfigure.6.1}{}}
\newlabel{fig:small_po@cref}{{[subfigure][1][6]6a}{[1][7][]8}{}{}{}}
\newlabel{fig:big_po}{{6b}{8}{Exploration of the shape index $p_0$. Panels (a, b): steady-state simulation snapshots centered on the channel obstacle for $p_0=3.2$ and $p_0=4.0$, respectively. Cells are rounder and more rigid at $p_0=3.2$, whereas they are considerably more deformable at $p_0=4.0$. Cell colors indicate asphericity ($\mathcal {A}$). The inset within the obstacle shows a magnified view of a selected square region of the tissue. Panel (c): effect of cell deformability parameter $p_0$ on tissue velocity ($v_{\uparrow }$) and mean asphericity over all membranes in the channel ($\langle \mathcal {A} \rangle $). Both $v_{\uparrow }$ and $\langle \mathcal {A} \rangle $ increase monotonically with increasing $p_0$, demonstrating that more flexible cells enable faster collective migration through the channel. Error bars represent the standard error of the mean. Panel (d): asphericity distribution ($p(\mathcal {A})$) for all membranes in the channel at the final state, shown for three values of $p_0$. At lower $p_0$, the membranes are predominantly circular, resulting in a pronounced peak at $\mathcal {A}=0$. As $p_0$ increases, the distribution broadens toward larger $\mathcal {A}$, indicating increasingly elongated membrane shapes}{subfigure.6.2}{}}
\newlabel{fig:big_po@cref}{{[subfigure][2][6]6b}{[1][7][]8}{}{}{}}
\newlabel{fig:po_exploration}{{6c}{8}{Exploration of the shape index $p_0$. Panels (a, b): steady-state simulation snapshots centered on the channel obstacle for $p_0=3.2$ and $p_0=4.0$, respectively. Cells are rounder and more rigid at $p_0=3.2$, whereas they are considerably more deformable at $p_0=4.0$. Cell colors indicate asphericity ($\mathcal {A}$). The inset within the obstacle shows a magnified view of a selected square region of the tissue. Panel (c): effect of cell deformability parameter $p_0$ on tissue velocity ($v_{\uparrow }$) and mean asphericity over all membranes in the channel ($\langle \mathcal {A} \rangle $). Both $v_{\uparrow }$ and $\langle \mathcal {A} \rangle $ increase monotonically with increasing $p_0$, demonstrating that more flexible cells enable faster collective migration through the channel. Error bars represent the standard error of the mean. Panel (d): asphericity distribution ($p(\mathcal {A})$) for all membranes in the channel at the final state, shown for three values of $p_0$. At lower $p_0$, the membranes are predominantly circular, resulting in a pronounced peak at $\mathcal {A}=0$. As $p_0$ increases, the distribution broadens toward larger $\mathcal {A}$, indicating increasingly elongated membrane shapes}{subfigure.6.3}{}}
\newlabel{fig:po_exploration@cref}{{[subfigure][3][6]6c}{[1][7][]8}{}{}{}}
\newlabel{fig:pa_exploration}{{6d}{8}{Exploration of the shape index $p_0$. Panels (a, b): steady-state simulation snapshots centered on the channel obstacle for $p_0=3.2$ and $p_0=4.0$, respectively. Cells are rounder and more rigid at $p_0=3.2$, whereas they are considerably more deformable at $p_0=4.0$. Cell colors indicate asphericity ($\mathcal {A}$). The inset within the obstacle shows a magnified view of a selected square region of the tissue. Panel (c): effect of cell deformability parameter $p_0$ on tissue velocity ($v_{\uparrow }$) and mean asphericity over all membranes in the channel ($\langle \mathcal {A} \rangle $). Both $v_{\uparrow }$ and $\langle \mathcal {A} \rangle $ increase monotonically with increasing $p_0$, demonstrating that more flexible cells enable faster collective migration through the channel. Error bars represent the standard error of the mean. Panel (d): asphericity distribution ($p(\mathcal {A})$) for all membranes in the channel at the final state, shown for three values of $p_0$. At lower $p_0$, the membranes are predominantly circular, resulting in a pronounced peak at $\mathcal {A}=0$. As $p_0$ increases, the distribution broadens toward larger $\mathcal {A}$, indicating increasingly elongated membrane shapes}{subfigure.6.4}{}}
\newlabel{fig:pa_exploration@cref}{{[subfigure][4][6]6d}{[1][7][]8}{}{}{}}
\newlabel{sec:po_exploration}{{7}{9}{Membrane deformability promotes shape elongation and faster tissue flow}{section.7}{}}
\newlabel{sec:po_exploration@cref}{{[section][7][]7}{[1][9][]9}{}{}{}}
\newlabel{tensor_gir}{{11}{9}{Membrane deformability promotes shape elongation and faster tissue flow}{equation.11}{}}
\newlabel{tensor_gir@cref}{{[equation][11][]11}{[1][9][]9}{}{}{}}
\newlabel{comp_gir}{{12}{9}{Membrane deformability promotes shape elongation and faster tissue flow}{equation.12}{}}
\newlabel{comp_gir@cref}{{[equation][12][]12}{[1][9][]9}{}{}{}}
\newlabel{asphericity}{{13}{9}{Membrane deformability promotes shape elongation and faster tissue flow}{equation.13}{}}
\newlabel{asphericity@cref}{{[equation][13][]13}{[1][9][]9}{}{}{}}
\newlabel{sec:comp_exp}{{8}{9}{Comparison with experiment}{section.8}{}}
\newlabel{sec:comp_exp@cref}{{[section][8][]8}{[1][9][]9}{}{}{}}
\newlabel{tab:axis_def}{{4}{9}{Definition of axes used for velocity profile comparison. $R$ is the obstacle radius}{table.caption.11}{}}
\newlabel{tab:axis_def@cref}{{[table][4][]4}{[1][9][]9}{}{}{}}
\newlabel{fig:exp_comp_ref_x}{{7a}{10}{\relax }{figure.caption.10}{}}
\newlabel{fig:exp_comp_ref_x@cref}{{[subfigure][1][7]7a}{[1][9][]10}{}{}{}}
\newlabel{sub@fig:exp_comp_ref_x}{{a}{10}{\relax }{figure.caption.10}{}}
\newlabel{sub@fig:exp_comp_ref_x@cref}{{[subfigure][1][7]7a}{[1][9][]10}{}{}{}}
\newlabel{fig:exp_comp_ref_y}{{7b}{10}{\relax }{figure.caption.10}{}}
\newlabel{fig:exp_comp_ref_y@cref}{{[subfigure][2][7]7b}{[1][9][]10}{}{}{}}
\newlabel{sub@fig:exp_comp_ref_y}{{b}{10}{\relax }{figure.caption.10}{}}
\newlabel{sub@fig:exp_comp_ref_y@cref}{{[subfigure][2][7]7b}{[1][9][]10}{}{}{}}
\newlabel{fig:exp_comp_ref}{{7}{10}{Comparison of velocity profiles between simulation and experiment along the axes illustrated in the graph at the bottom left corner of panel (\subref {fig:exp_comp_ref_x}). Data points with symbols (crosses, squares, circles, etc.) represent experimental measurements, while solid or dashed lines correspond to simulation results. Panel \subref {fig:exp_comp_ref_x} displays the $x$-component of velocity along the axes, and panel \subref {fig:exp_comp_ref_y} shows the $y$-component. All velocities are normalized by the downstream velocity ($v_{\downarrow }$), as defined in the text, and the length along the axis is given in units of the obstacle radius $R$. Overall, there is good agreement between simulation and experiment: in most cases, the simulated curves lie within the range of the experimental data (the shaded region). The main exceptions occur at the beginning of axes $1$, $2a$, and $2b$, which we attribute to experimental limitations in establishing a steady flow. The simulated curves for the vertical axes ($3$, $4$, and $5$) extend slightly further than the experimental curves because the spatial window used to generate the velocity field in the experiment is larger than that used in the simulations. In the simulations, a smaller spatial window could be used due to the larger time average available}{figure.caption.10}{}}
\newlabel{fig:exp_comp_ref@cref}{{[figure][7][]7}{[1][9][]10}{}{}{}}
\newlabel{LastPage}{{9}{13}{}{page.13}{}}

